The Rise of Disappearing Frameworks in Web Development

The evolution of the web can be characterized as an emergence of frameworks paving the way from static websites to dynamic web applications. As the scope of web applications has grown, new technical challenges have emerged, leading to the need for new solutions. The latest of these developments is the rise of so-called disappearing web frameworks that question the axioms of earlier generations of web frameworks, providing benefits of the early web and simple static sites.

==> 10-astro.tex <==
Astro\footnote{\url{https://astro.build/}} is a static site generator (SSG) built with the islands architecture in mind. It could be characterized rather as a build tool than a framework given it has been designed to work with many of the existing frameworks instead of being an option to them \cite{whatisastro}. The goal of the project is to allow developer experience (DX) familiar from contemporary frameworks but within a static environment \cite{whatisastro}. Astro achieves this in a several ways:

\begin{enumerate}
    \item Islands are supported out of the box - In other words, developers can decide which component boundaries should be interactive. \cite{astrodocs}
    \item Server-first API design - To minimize the cost of hydration, work is offloaded to the server as possible. \cite{astrodocs}
    \item Zero JavaScript by default - Astro doesn't emit any JavaScript by default. \cite{astrodocs}
    \item Edge-ready - Astro sites can be deployed anywhere, edge included, due to its static nature. \cite{astrodocs}
    \item Customizable - Numerous extensions exist to expand the capabilities of Astro. \cite{astrodocs}
    \item UI-agnostic - Astro can act as a host for many of the contemporary JavaScript frameworks. \cite{astrodocs}
\end{enumerate}

% astrodocs - https://docs.astro.build/en/getting-started/
% whatisastro - https://javascript.plainenglish.io/what-is-astro-aa3369d5a7f4
% introtoastro - https://www.infoworld.com/article/3669877/intro-to-astro-clever-lazy-loading-for-javascript.html

\subsection{Astro islands}

TODO

\subsection{Server-first API design}

TODO

\subsection{Customizability}

TODO

\subsection{Conclusion}

TODO


==> 11-marko.tex <==
Marko\footnote{\url{https://markojs.com/}}

eBay + their requirements

compiler-based approach

https://www.infoworld.com/article/3643329/hands-on-with-the-marko-javascript-framework.html

\subsection{Conclusion}

TODO


==> 12-qwik.tex <==
% TODO: https://www.builder.io/blog/movies-app-in-7-frameworks-which-is-fastest-and-why

Qwik\footnote{\url{https://qwik.builder.io/}} is a web framework built by Miško Hevery (Angular.js), Adam Bradley (Ionic), and Manu Almeida (Gin Framework) \cite{adservioQwikPostModern}. The framework addresses the conflicting requirements of interactivity and page speed \cite{devmQwiksMagic}. The conflict means you have to compromise in either interactivity or speed due to the hydration cost of the current frameworks \cite{devmQwiksMagic}. According to Qwik documentation \cite{qwikdocs}, the framework is solving the quandary using the following means:

\begin{enumerate}
    \item Resumability over hydration - Instead of hydrating, Qwik can resume code execution on demand.
    \item Automatic code splitting - Due to the approach, Qwik splits code aggressively, meaning the developer does not have to perform manual effort like with the other frameworks.
    \item Tiny runtime - The size of Qwik runtime is only one kilobyte.
    \item Compilation over runtime cost - Qwik has an optimizer achieving the above and pushing some state management to the server side.
\end{enumerate}

It is these factors that make Qwik unique compared to its competition. Qwik is consistent with the idea of disappearing frameworks, discussed in the Section \ref{sec:disappearing-frameworks}, as it tries to make itself vanish from the application. Because of its approach, Qwik represents a paradigm-level shift in how to develop web applications. One of the ways it achieves its targets is by focusing on different metrics than its predecessors, namely Time to Interactive (TTI)\footnote{By Time to Interactive (TTI), we mean the amount of time it takes for a webpage to become interactive from the perspective of the user.} over Time to Load (TTL)\footnote{By Time to Load (TTL), we mean the amount of time it takes for a page to load from the perspective of the web browser. Compared to TTI, the page isn't interactive yet by then since the browser still has to evaluate the code that was loaded.}.

While many frameworks focus on TTL, the core metric of Qwik is TTI \cite{infoworldIntroQwik}. The developers of Qwik are concerned about how soon a web page can become responsive to user interaction. It is this shift in perspective that likely motivated the approach and the idea of resumability.

\subsection{Resumability}

Resumability allows pages to become interactive on demand based on user intent \cite{devmQwiksMagic} while picking up where the server left off \cite{adservioQwikPostModern}. In contrast to hydration-based approaches, there is less work to do for the browser as a part of it has been performed already. As a result, TTI can become low and the page can become responsive to the user interaction fast.

The idea of resumability is not new as illustrated by the example of jQuery (2006) \cite{devmQwiksMagic}. The difference to jQuery is that working with Qwik is similar to working with React in terms of developer experience (DX) as it has adopted a similar component style and supports reactive state management out of the box \cite{devmQwiksMagic}. To leverage resumability, Qwik generates both server and client-side code while serializing using a so-called optimizer \cite{devmQwiksMagic}

\subsection{Optimizer and automatic code splitting}

The optimizer is a core part of Qwik generating code using automatic code splitting applied across component and event listeners, meaning Qwik defers loading necessary code as long as possible \cite{qwikresumability}. Given deferring isn't always the preferred behavior, Qwik supports standard preloading strategies \cite{qwikresumability}. The strategies are then used by a service worker set up by Qwik to monitor application state \cite{devmQwiksMagic}.

For code splitting, Qwik has been split architecturally into three parts \cite{devYourBundler}: view, state, and handlers. Usually, these three parts are coupled and held together in code. The coupling means there are three parts to download, parse, and execute together \cite{devYourBundler}. Even if only one part is needed based on user interaction, all three need to be processed regardless \cite{devYourBundler}.

Because of the separation of concerns, in Qwik automatic code splitting has become possible at an unprecedented level. To mark the code splitting boundaries, a specific dollar based code convention is used, and then the optimizer can compile the code based on them \cite{qwikdocs}. Due to the shift in perspective, Qwik can achieve fine-grained code splitting out of the box that its predecessors couldn't due to their tighter coupling of concerns.

\subsection{Code splitting boundaries, reactive state, and components}

To get a better idea of how code splitting boundaries work in Qwik, consider the counter-based example below from Qwik documentation \cite{qwikdocs}. It also illustrates the usage components and reactive state of Qwik\footnote{In technical terms, Qwik's state manager has been built on top of proxies. \cite{qwikdocs}}.

\begin{lstlisting}[language=javascript]
import { component$, useStore } from '@builder.io/qwik';

export default component$(() => {
  const store = useStore({ count: 0 });

  return (
    <div>
      <span>Count: {store.count}</span>
      <button onClick$={() => store.count++}>Click</button>
    </div>
  );
});
\end{lstlisting}

It is good to note that the example is fairly close to the code you would write in React. As a pioneer, React created good programming interfaces, and Qwik decided to mimic them while adding its twists on top.

As a downside of code splitting, Miško Hevery mentions Qwik has to ensure the code is ready before the interaction to avoid delays from the user point of view \cite{devmQwiksMagic}. For this purpose, Qwik utilizes a service worker\footnote{\href{https://developer.mozilla.org/en-US/docs/Web/API/Service_Worker_API}{Service Worker} is a standard web API that allows building proxy servers between the server and the client. In other words, using the technology, you can intercept client traffic and shape it.}.

% Miško Hevery describes the technical challenge of Qwik as "death by closure" \cite{infoworldIntroQwik}. In a conventional approach, the application would need to maintain all its state consistently at the root level and share it with the consumers from there. In Qwik, a global event listener is used instead, and the listener's responsibility is to orchestrate the registration of event handlers as they are loaded on demand \cite{infoworldIntroQwik}.

\subsection{Qwik City}

Qwik City\footnote{\url{https://qwik.builder.io/qwikcity/overview/}} is a meta-framework comparable to Next.js for React \cite{devmQwiksMagic}. It provides the following features on top of Qwik \cite{devmQwiksMagic}:

\begin{itemize}
    \item Directory-based routing
    \item Nested layouts
    \item File-based menus
    \item Breadcrumbs
    \item Support authoring content with .tsx or .mdx file formats
    \item Data endpoints
\end{itemize}

In addition, Qwik City comes with Partytown\footnote{\url{https://partytown.builder.io/}}, a technical solution running third-party scripts in a web worker, thereby speeding up the website by avoiding main thread congestion. Congestion can occur when third-party scripts compete with application code. Such scripts are often related to web analytics or e-commerce, for example.

The technical target of Qwik City is to provide the capabilities of a multi-page application (MPA) with the benefits of a single page application (SPA) \cite{devmQwiksMagic}. Therefore navigation-wise, the solution avoids page refreshes commonly encountered in MPAs and allows user experience (UX) familiar from SPAs.

\subsection{Observations}

Qwik represents a paradigm-level shift in how web applications are developed. It approaches the problem from a different angle and compared to earlier solutions, it tries to solve the issue of providing highly interactive pages to the client fast on a tooling level thanks to its compiler-based implementation. At the same time, it has adopted ergonomics familiar to developers from earlier frameworks, mainly React, easing its adoption.

\begin{comment}
\subsection{Solid.js}

reactive by default

https://www.infoworld.com/article/3643331/hands-on-with-the-solid-javascript-framework.html

https://www.infoworld.com/article/3626348/solidjs-creator-javascript-innovation-isnt-slowing-down.html

https://blog.openreplay.com/alternatives-to-react-solid-js

\subsection{Gustwind}

built around JSON

more like a set of guidelines

I might even leave this out and develop further (another paper by itself)

\subsection{Comparison}

TODO: some table here with compilation, paradigm etc.
\end{comment}

==> 13-current-trends.tex <==
TODO

\subsection{The current front-end development landscape}

The current front-end development landscape is dominated by React, Vue, and Angular\footnote{Based on Stack Overflow Survey of 2022 \cite{soSurvey2022}, 42.62\% of developers use React. For Angular, the figure was 20.39\%, and for Vue 18.82\%. W3Techs \cite{w3techsReactVuejs2022} puts these values into perspective as there the global market share of React is around 3.7\% for all websites.}. Furthermore, solutions such as Next.js or Nuxt.js\footnote{Based on \cite{soSurvey2022}, 13.52\% of developers use Next.js so that means roughly one out of four React developers use Next.js. For Nuxt.js, the figure is 3.83\% which means roughly one out of six.}, have been built on top of these to add more structure and opinions. Each of the contemporary solutions relies on several key ideas we've listed below:

\begin{enumerate}
    \item Component orientation -- They come with component-oriented abstractions\footnote{By these, we mean a way to encapsulate markup and potentially local state so that it can be reused.}
    \item Templating -- A solution, such as JSX, is used for modeling markup
    \item Hydration -- To make the components come alive, the solutions run the code at the client side. By this, we mean attaching event handlers and running component logic \cite{huotala2021benefits}.
\end{enumerate}

Depending on the flavor, you can see different technical implementations for each concern. Overall, the core ideas tend to be the same. Regardless of the approach, the solutions rely on a runtime the client has to load before running any application code.

% To understand the technical concerns better, we discuss the main ideas in detail in the following sections before addressing the limitations of the contemporary approaches as those motivate the development of new solutions, which we cover in the next section of the paper.

\subsection{Conclusion}

TODO

